Leadership in Singleton Congestion Games: What is Hard and What is Easy

We study the problem of computing Stackelberg equilibria Stackelberg games whose underlying structure is in congestion games, focusing on the case where each player can choose a single resource (a.k.a. singleton congestion games) and one of them acts as leader. In particular, we address the cases where the players either have the same action spaces (i.e., the set of resources they can choose is the same for all of them) or different ones, and where their costs are either monotonic functions of the resource congestion or not. We show that, in the case where the players have different action spaces, the cost the leader incurs in a Stackelberg equilibrium cannot be approximated in polynomial time up to within any polynomial factor in the size of the game unless P = NP, independently of the cost functions being monotonic or not. We show that a similar result also holds when the players have nonmonotonic cost functions, even if their action spaces are the same. Differently, we prove that the case with identical action spaces and monotonic cost functions is easy, and propose polynomial-time algorithm for it. We also improve an algorithm for the computation of a socially optimal equilibrium in singleton congestion games with the same action spaces without leadership, and extend it to the computation of a Stackelberg equilibrium for the case where the leader is restricted to pure strategies. For the cases in which the problem of finding an equilibrium is hard, we show how, in the optimistic setting where the followers break ties in favor of the leader, the problem can be formulated via mixed-integer linear programming techniques, which computational experiments show to scale quite well.

==> algorithms_same_actions_ijcai.tex <==
\section{SSSCGs with Arbitrary Costs -- IJCAI Version}\label{sec:algorithms_same_actions_general_costs_ijcai}

\todo{This is the IJCAI section, it must be replaced.}

Finally, let us shift our attention to general SSSCGs, i.e., games in which the costs need not be monotonic functions of the resource congestion.

\begin{observation}
	Given an SSSCG, an optimal leader's pure strategy to commit to can be computed efficiently, both in the optimistic and the pessimistic case.
\end{observation}

Clearly, when the followers' costs are monotonic functions, we can find an optimal leader's pure strategy using Algorithm~\ref{algorithm}.
%
In general, we can apply a procedure similar to that of Algorithm~\ref{algorithm}, enumerating the leader's pure strategies while computing, for each of them, an NE minimizing/maximizing the leader's cost in the resulting followers' game.
%
In order to find one such NE, we can adapt an algorithm proposed in~\cite{ieong2005fast}, which relies on dynamic programming to compute in $O(r^5 n^6)$ an NE minimizing the social-cost in SSSCGs without leadership.
%
It suffices to change the objective function from the social cost to the leader's cost of the resource selected in the current pure strategy.
%
Thus, in general, the overall computation requires $O(r^6 n^6)$.

Unfortunately, the assumption that the leader always plays pure strategies is not safe in SSSCGs with arbitrary costs, as Theorems~\ref{thm:pure_strategy_opt}~and~\ref{thm_pure_strategies_pes} do not hold if the monotonicity assumption is dropped.

\begin{observation}
	There are SSSCGs such that:
	\begin{itemize}[nolistsep,itemsep=0mm]
		\item the followers' costs only are non-monotonic, and any O/PSE prescribes the leader to play a mixed strategy;
		\item the leader's costs only are non-monotonic, and any O/PSE prescribes the leader to play a mixed strategy.
	\end{itemize}
\end{observation}

Consider a game with a single follower, $R =\{ r_1, r_2 \}$, and players' costs as in Figure~\ref{fig:ex_games}(c).
%
Clearly, the follower selects $r_2$ whenever $\sigma_\ell(r_1) \leq \frac{1}{2}$, while, if $\sigma_\ell(r_1) \geq \frac{1}{2}$, she chooses $r_1$, providing the leader with a cost of $2 - \sigma_\ell(r_1)$ and $1 + \sigma_\ell(r_1)$, respectively.
%
Thus, any O/PSE prescribes the leader to play $\sigma_\ell$ such that $\sigma_\ell(r_1) = \frac{1}{2}$.

Moreover, when the players' costs are as in Figure~\ref{fig:ex_games}(d), the follower selects $r_2$ if $\sigma_\ell(r_1) \geq \frac{1}{2}$, and $r_1$ if $\sigma_\ell(r_1) \leq \frac{1}{2}$, providing the leader with a cost of $2 \sigma_\ell(r_1)$ and $2 - 2 \sigma_\ell(r_1)$, respectively.
%
As a result, any O/PSE of the game prescribes the leader to play $\sigma_\ell$ such that $\sigma_\ell(r_1) = \frac{1}{2}$.

